Open/closed string duality and relativistic fluids

We propose an open/closed string duality in general backgrounds extending previous ideas about open string completeness by Ashoke Sen. Our proposal sets up a general version of holography that works in gravity as a tomographic principle. We argue, in particular, that previous expectations of a supergravity/Dirac-Born-Infeld (DBI) correspondence are naturally embedded in this conjecture and can be tested in a well-defined manner. As an example, we consider the correspondence between open string field theories on extremal D-brane setups in flat space in the large-N, large 't Hooft limit, and asymptotically flat solutions in ten-dimensional type II supergravity. We focus on a convenient long-wavelength regime, where specific effects of higher-spin open string modes can be traced explicitly in the dual supergravity computation. For instance, in this regime we show how the full abelian DBI action arises from supergravity as a straightforward reformulation of relativistic hydrodynamics. In the example of a (2+1)-dimensional open string theory this reformulation involves an abelian Hodge duality. We also point out how different deformations of the DBI action, related to higher-derivative corrections and non-abelian effects, can arise in this context as deformations in corresponding relativistic hydrodynamics.

==> hyperbasics.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                         %
% This file is written by Tanmoy Bhattacharya <tanmoy@qcd.lanl.gov> and   %
% is in the public domain for what it is worth. It inserts \specials that %
% are interpreted by (a) the xhdvi hypertex dvi previewer, (b) nextstep   %
% HyperTeXview.app dvi previewer, and (c) the dvipdf driver               %
% For more info, see http://xxx.lanl.gov/hypertex/                        %
%                or  ftp://xxx.lanl.gov/pub/hypertex/index.html           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                         %
% Only \hyperdef, \hyperref , \href , and \hname are user callable.       %
% Usage: \hyperdef\TeXcs{category}{name}{text}                            %
% Usage: \href{url}{text}                                                 %
% Usage: \hyperref{filename}{category}{name}{text}                        %
%   or   \hyperref\TeXcs{text}                                            %
%             where \TeXcs has been defined by a hyperdef.                %
%                                                                         %
%        Note: The token following \hyperref is expanded completely first.%
%              Really perverse forms like                                 %
%                \csname perverse\endcsname                               %
%              will give an error                                         %
%                                                                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following might be useful to other macros interfacing in.           %
% Usage: \hyper@nchor{name="#myname" href="#refer"}{text}                 %
% Usage: \hyperlink{target_name}{text}                                    %
% Usage: \hypertarget{myname}{text}                                       %
% In cases where there is a possibility of premature expansion use        %
%     \hyper@\hyperpr@ref instead of \hyperref                            %
% and \hyper@\hyperpr@def instead of \hyperdef                            %
% These macros increase enormously in size when expanded, but the expanded%
% token sequence always ends in \hyperpr@ref and \hyperpr@def respectively%
% Macro writers might want to make use of the macro \hyperv@rsion         %
% which is undefined in version 0 and is the version number otherwise     %
% \hyper@nique is exactly like \hyperdef except no special are written    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Save the current catcode of @ and redefine @ to be a letter
%
\expandafter\edef\csname hypers\string @fe\endcsname{\catcode
                                             `\noexpand @=\the\catcode`\@}%
\catcode`\@=11
%
% Check if the file is already included
%
% hack to allow \allowoncemore
\ifx\hyper@utoprocess\hyper@ndefined
\else
 \expandafter\hyper@utoprocess\fi
\ifx\hyperd@ne\hyper@ndefined
 \global\let\hyperd@ne=\relax
\else
 \hypers@fe
 \errhelp{hyperbasics.tex needs to be included only once outside
          of any {...} or \begingroup...\endgroup. You have tried to
          include it more than once. If the previous include was indeed
          outside any groupings, continue and all will be well.}%
 \errmessage{Input this file only once!}%
 \expandafter\endinput\fi
%
% Version number
%
\def\hyperv@rsion{12}%
%
% Check and input a previous .hrf file if it exists
%
\newread\hyperf@le
\def\hyperf@lename{\jobname.hrf}%
\immediate\openin\hyperf@le\hyperf@lename\relax
\ifeof\hyperf@le\relax
 \immediate\closein\hyperf@le\relax
\else
 \immediate\closein\hyperf@le\relax
 \input \hyperf@lename
\fi
%
% Open a new .hrf file
%
\newwrite\hyperf@le
\immediate\openout\hyperf@le\hyperf@lename
%%%%
% MAIN SECTION
%%%%
%
% define a token register
%
\newtoks\hypert@ks
%
% Define a convenient macro to hold the character #
%
\edef\hypert@mp{\catcode`\noexpand\%=\the\catcode`\%}
\catcode`\%=12
\def\hyperp@rcent{%}
\hypert@mp
\edef\hypert@mp{\catcode`\noexpand\#=\the\catcode`\#}%
\catcode`\#=12
\def\hyperh@sh{#}%
\hypert@mp
\let\hypert@mp=\relax
\let\hyper@nd=\relax
\def\hyperbl@nk{ }
\def\hyperstr@pquote#1"#2\hyper@nd{% Call \hyperstr@pquote..."\hyper@nd
   #1% #1 can not contain "
   \ifx\hyper@nd#2\hyper@nd% #2 cannot contain \hyper@nd and
                           % must end in " if non-empty
   \else\hyperp@rcent22\hyperstr@pquote#2\hyper@nd\fi}%
\def\hyperstr@pblank#1 #2\hyper@nd{% Call \hyperstr@pblank... \hyper@nd
   #1% #1 cannot contain a space
   \ifx\hyper@nd#2\hyper@nd% #2 canot contain \hyper@nd and
                           % and must end in blank if nonempty
   \else\hyperp@rcent20\hyperstr@pblank#2\hyper@nd\fi}
%
\long\def\hyper@nchor#1#2{\edef\hyperm@cro{html:<A #1>}%
                          \special\expandafter{\hyperm@cro}%
                          {#2}\special{html:</A>}}%
%
\def\hyper@atm@ning#1->#2\hyper@nd{#2}
\def\hyperlink{\protect\hyperlink@}
\def\hyperlink@{{\catcode\expandafter`\noexpand\#=12 
                 \catcode\expandafter`\noexpand\%=12 
                 \catcode\expandafter`\noexpand\~=12
                \expandafter}\hyperlink@@}
\def\hyperlink@@#1{\protect\hyperlink@@@{#1}}
\def\hyperlink@@@#1{\edef\hypert@mp{#1}%
               \edef\hypert@mp{\expandafter\hyper@atm@ning\meaning\hypert@mp
                               \hyper@nd}%
               \edef\hypert@mp{\expandafter\hyperstr@pquote%
                               \hypert@mp"\hyper@nd}%
               \edef\hypert@mp{\expandafter\expandafter\expandafter
                               \hyperstr@pblank\expandafter%
                               \hypert@mp\hyperbl@nk\hyper@nd}%
               \hyper@nchor{href=\expandafter"\hypert@mp"}}%
%
\def\hypertarget#1{\edef\hypert@mp{#1}%
               \edef\hypert@mp{\expandafter\hyper@atm@ning\meaning\hypert@mp
                               \hyper@nd}%
               \edef\hypert@mp{\expandafter\hyperstr@pquote%
                               \hypert@mp"\hyper@nd}%
               \edef\hypert@mp{\expandafter\expandafter\expandafter
                               \hyperstr@pblank\expandafter%
                               \hypert@mp\hyperbl@nk\hyper@nd}%
               \hyper@nchor{name=\expandafter"\hypert@mp"}}%
%
\def\hyperref{\afterassignment\hyperr@f\let\hyperp@ram}
\def\hyperr@f{\ifx\hyperp@ram{\iffalse}\fi
               \expandafter\expandafter\expandafter\hyperr@@
               \expandafter{%
              \else
               \iffalse}\fi
               \ifx\hyperp@ram\hyper@ndefined
                 \message{Undefined reference}%
                 \def\hyperp@r@m{{}{undefined}{}}%
               \else
                 \edef\hyperp@r@m{\hyperp@ram}%
               \fi
               \expandafter\expandafter\expandafter\hyperr@@
               \expandafter\hyperp@r@m
              \fi}%
% refer to #1, \hyperh@sh#2.#3 or #1\hyperh@sh#2.#3
% depending on what is blank/nonblank
\def\hyperr@@#1#2#3{\ifx\hyper@ndefined#1\hyper@ndefined
                    \hypert@ks\expandafter{\hyperh@sh#2.#3}%
                    \else
                     \ifx\hyper@ndefined#2#3\hyper@ndefined
                      \hypert@ks{#1}%
                     \else
                      \def\hypert@mp{#1}%
                      \hypert@ks\expandafter\expandafter\expandafter
                      {\expandafter\hypert@mp\hyperh@sh#2.#3}%
                     \fi
                    \fi
                    \expandafter\hyperlink\expandafter{\the\hypert@ks}}%
%
% \def\hyperREF#1{\hyperlink{#1}}% % Disabled as per pg's suggestion
%
\def\hyperdef#1#2#3{{\escapechar=`\\\relax
                     \edef\hyper@t@mp@{\hyperstr@pquote#2.#3"\hyper@nd}%
                     \expandafter\ifx\csname hyperd@\meaning\hyper@t@mp@
                     \endcsname
                     \relax
                     \expandafter\gdef\csname hyperd@\meaning\hyper@t@mp@
                     \endcsname{}%
                     \gdef#1{{}{\hyperstr@pquote#2"\hyper@nd}%
                               {\hyperstr@pquote#3"\hyper@nd}}%
                     \immediate\write\hyperf@le{\def\noexpand#1{{}%
                        {\noexpand\hyperstr@pquote#2"\noexpand\hyper@nd}%
                        {\noexpand\hyperstr@pquote#3"\noexpand\hyper@nd}}}%
                     \xdef\hyper@t@mp@{\global\let\noexpand\hyper@t@mp@=\relax
                                       \noexpand\hypertarget{\hyper@t@mp@}}%
                     \global\hypert@ks={\hyper@t@mp@}%
                     \else
                     \message\expandafter{\expandafter'\hyper@t@mp@' duplicate}%
		     \def\hyper@@tmp@{\hyperdef{#1}{#2}}%
		     \edef\hyper@@tmp@@{{#3@}}%
                     \global\let\hyper@t@mp@=\relax
                     \global\hypert@ks=\expandafter\expandafter
		     \expandafter{\expandafter\hyper@@tmp@\hyper@@tmp@@}%
                     \fi}\the\hypert@ks}%

\def\hyper@nique#1#2#3#4{{\escapechar=`\\\relax
                     \edef\hyper@t@mp@{\hyperstr@pquote#2.#3"\hyper@nd}%
                     \expandafter\ifx\csname hyperd@\meaning\hyper@t@mp@
                     \endcsname
                     \relax
                     \gdef#1{{}{\hyperstr@pquote#2"\hyper@nd}%
                               {\hyperstr@pquote#3"\hyper@nd}}%
                     \global\let\hyper@t@mp@=\relax
                     #4%
                     \else
		     \def\hyper@@tmp@{\hyper@nique{#1}{#2}}%
		     \edef\hyper@@tmp@@{{#3@}}%
                     \global\let\hyper@t@mp@=\relax
   		     \expandafter\hyper@@tmp@\hyper@@tmp@@{#4}%
                     \fi}}%

%%% 
% protection macros
%%%
\ifx\protect\hyper@ndefined\let\protect=\relax\fi
\let\hyper@@@@=\relax
\def\hyper@@{\let\hyper@@@=\relax}%
\hyper@@
\def\hyper@{\relax\let\hyper@@@\noexpand\hyper@\noexpand}%
\def\hyperpr@ref{\hyper@@\hyperref}
\def\hyperpr@link{\hyper@@\hyperlink}
\def\hyperpr@def{\hyper@@\hyperdef}
\let\hyper@marker=\relax
\def\hyper@@tokenize#1\hyper@marker{#1}
\def\hyper@tokenize{\expandafter\endgroup\hyper@@tokenize}
\def\hyperpr@tokenize{\hyper@@\hyper@tokenize}

% As per pg's suggestion
\edef\href{\begingroup\catcode`\string @=11
            \hyper@\hyperpr@tokenize\hyper@\hyperpr@link
            \hyper@marker}
\let\hname\hypertarget
% Hack to allow auto-processing
\def\allowoncemore{\def\hyper@utoprocess{\let\hyper@utoprocess=\hyper@ndefined
                                         \hypers@fe\endinput}}%
%
% Restore the catcode of @
%
\hypers@fe
\endinput
% A line after endinput to avoid both msdos gremlins and an incomplete
% last line

